Large Scale Hierarchical Industrial Demand Time-Series Forecasting incorporating Sparsity

Hierarchical time-series forecasting (HTSF) is an important problem for many real-world business applications where the goal is to simultaneously forecast multiple time-series that are related to each other via a hierarchical relation. Recent works, however, do not address two important challenges that are typically observed in many demand forecasting applications at large companies. First, many time-series at lower levels of the hierarchy have high sparsity i.e., they have a significant number of zeros. Most HTSF methods do not address this varying sparsity across the hierarchy. Further, they do not scale well to the large size of the real-world hierarchy typically unseen in benchmarks used in literature. We resolve both these challenges by proposing HAILS, a novel probabilistic hierarchical model that enables accurate and calibrated probabilistic forecasts across the hierarchy by adaptively modeling sparse and dense time-series with different distributional assumptions and reconciling them to adhere to hierarchical constraints. We show the scalability and effectiveness of our methods by evaluating them against real-world demand forecasting datasets. We deploy HAILS at a large chemical manufacturing company for a product demand forecasting application with over ten thousand products and observe a significant 8.5\% improvement in forecast accuracy and 23% better improvement for sparse time-series. The enhanced accuracy and scalability make HAILS a valuable tool for improved business planning and customer experience.

==> Text/dump.tex <==

Leveraging distributional consistency error as a soft regularizer enforces forecast distributions to be well-calibrated
while adaptively adhering to the hierarchical relations of the dataset.
For the distance metric $\text{Dist}$ in Equation \ref{eqn:dce},
we use the Jensen-Shannon Divergence \cite{endres2003new} (JSD) as the distance metric since it is a symmetric
and bounded variant of the popularly used KL-Divergence distance.
Moreover, it assumes a closed form for many widely used distributions including for the Gaussian used in \profhit.
Due to parameterization
of each time-series distribution as a Gaussian we get a closed-form differentiable expression:
{\begin{equation}
    \begin{split}
        \mathcal{L}_{\text{dist}} &= \sum_{i=1}^N \frac{\refinedsigma_i^2 + \left( \refinedmu_i - \sum_{j\in C_i} \phi_{ij}\refinedmu_j \right)^2}{4\sum_{j\in C_i}\phi^2_{ij} \refinedsigma_j^2} +\\
        &\sum_{i=1}^N  \frac{\sum_{j\in C_i}\phi^2_{ij} \refinedsigma_j^2 + \left( \refinedmu_i - \sum_{j\in C_i} \phi_{ij}\refinedmu_j \right)^2}{4\refinedsigma_i^2} -\frac{1}{2}.
    \end{split}
    \label{eqn:jsd2}
\end{equation}}

Note that along with the SDCR loss $\mathcal{L}_{\text{dist}}$ which informs \model of hierarchical relations $H_\mathcal{T}$ optimizes for distributional consistency,
we derive the \textit{Likelihood Loss} $\mathcal{L}_{\text{ll}} = P(\{y_i^{(t+\tau)}\}_{i=1}^N| \mathcal{D}^t)$ to optimize for the accuracy and calibration of the forecasts.
Thus, the total loss for training is given as
$\mathcal{L} = \mathcal{L}_{\text{ll}} + \lambda \mathcal{L}_{\text{dist}}$
where the hyperparameter $\lambda$ controls the trade-off in importance between data likelihood and distributional consistency.

\subsection{Dealing with sparse (intermittent) time-series}

In our dataset, we observed that most time-series at the lower levels of the hierarchy
are sparse: most values of the time-series are zeroes with spikes in between. 
On average the bottom three levels of the hierarchy contain over 40\% of values as
zeroes in time-series.
Therefore, standard models which forecast on real-values with smoother time-series
may not model these patterns well with the default Gaussian distribution.
Therefore, we modify \profhit to enable it to model these sparse time-series 
at a lower level. We propose two methods for tackling this issue.



%\begin{figure}[h]
%    \centering
%    \includegraphics[width=.8\linewidth]{Images/SparseRetrofit.png}
%    \caption{Retrofitting Sparse models (e.g.: LightGBM) with \profhit}
%    \label{fig:sparse-retrofit}
%\end{figure}

\paragraph{Retrofitting \profhit for sparse time-series models}
\profhit was originally designed to model forecasts as Gaussian distributions
which are apt for dense real-valued time-series. However, 
they may fail on sparse data at lower levels.
Therefore, we propose using models specific to sparse time-series such as LightGBM~\cite{ke2017lightgbm}
or Croston model~\cite{croston1972forecasting}.

We retrofit the sparse model used to forecast the lower levels of the hierarchy
with \profhit used for higher levels to enable
exchange of information across the hierarchy and to provide coherent forecasts. 
We do this via a two-step integration method (see Figure \ref{fig:sparse-retrofit}):
\begin{itemize}
    \item \textbf{Top-bottom integration:} Empirically we observe that the accuracy of the
    forecasts at higher levels by \profhit is more accurate than at lower levels.
    Therefore, we use the forecasts from the higher level of the hierarchy as additional
    features to the sparse forecasting model.
    \item \textbf{Bottom-top integration:} We directly use the predictions of the
    lower levels models in the SDCR loss to train the parameters of \profhit.
    This enables \profhit to provide forecasts that are hierarchically coherent
    with the sparse-model forecasts.
\end{itemize}

\paragraph{Modeling sparse time-series with Poisson Distribution}
Instead of using Gaussian parameters, we use a Poisson distribution for each of the 
lower level nodes with GRU output for node $i$ as parameter $\lambda_i$.
A Poisson distribution can model cases where the samples can be zero or low valued with high probability.
The base forecast parameters for lower levels are therefore 
$\lambda = [\lambda_1, \dots, \lambda_K]$ and the refinement module 
refines these parameters similar to
Gaussian means:
\begin{equation}
    \gamma_i = \text{sigmoid}(\hat{w}_i), \quad
    \refinedlambda_i = \gamma_i \lambda_i + (1-\gamma_i) \mathbf{w}_i^T\mathbf{\lambda}.
    \label{eqn:corempoisson}
\end{equation}


To calculate the SDCR between lower levels of the hierarchy (both of which are Poisson) is straightforward since (similar to a Gaussian distribution), the Poisson distribution also has
a closed-form solution for JSD distance:
\begin{equation}
    JSD(\lambda_1, \lambda_2) = \lambda_1 \log\left(\frac{\lambda_1}{\lambda_2}\right)
    + \lambda_2 \log\left(\frac{\lambda_2}{\lambda_1}\right).
\end{equation}

However, as we go higher up the hierarchy, the summation of lower-level Poisson distributions  
makes the time-series less sparse and therefore more amenable to modeling
using a Gaussian distribution which can independently model the mean and variance
of the distribution allowing for better calibration for smoother higher-level time-series.
We leverage the central limit theorem to approximate the sum of Poisson distribution
as Gaussian as follows:
\begin{theorem}
    Let $X_1, X_2, \dots, X_N$ be $N$ independent Poisson random variables with
    parameters $\lambda_1, \lambda_2, \dots, \lambda_N$. 
    Then denote $Y$ as $Y=\sum_{i=1}^N X_i$. Then $Y$ is a Poisson variable with
    parameter $\lambda_Y = \sum_{i=1}\lambda_i$.
    Then for sufficiently large $\lambda_Y$, $Y$ can be approximated by a
    Gaussian distribution $\Tilde{Y} = \mathcal{N}(\lambda, \sqrt{\lambda})$~\cite{PoissonN28:online}.
\end{theorem}
Therefore, from the fourth level and above we can approximate the sum of Poisson variables of children as a Gaussian distribution and use Equation ~\ref{eqn:jsd2} to calculate SDCR for these levels.

\subsection{Faster training via Asynchronous model updates}
\label{sec:async}

\begin{figure}[h]
    \centering
    \includegraphics[width=.7\linewidth]{Images/Async.png}
    \caption{Asynchronous Updates of two modules of \profhit.
    Reconciliation module is more frequently updated where the larger
    base forecasting models are updated with less frequency.}
    \label{fig:async}
\end{figure}

Training base forecasting models for over 10,000 time-series is very time and compute
intensive, especially when dealing with large parameterized deep-learning models.
However, the hierarchy reconciliation model doesn't have many parameters
and can be trained frequently.
To facilitate efficient overall training by enabling the
reconciliation module to better refine the forecast, we train the two modules
of \profhit with different frequency.
We update the gradients of the reconciliation module for every batch where
as we update the base-forecasting modules for every
node of the hierarchy for every $K$ batches where $K$ is a hyperparameters.
This enables \model to learn to better reconcile more frequently while
not overtraining the base forecasting model for every node (see Figure ~\ref{fig:async}).

\subsection{Visualization Functionality and Improvements}

\paragraph{Motivation}
Analyzing over 20 thousand forecasts over the entire demand hierarchy is non-trivial.
To evaluate the efficacy of our forecasts as well as compare them against other models' predictions 
requires a suite of visualization tools that can aid data analysts and decision-makers
answer crucial questions and gain important insights.
Therefore, we design a set of interactive visualization tools aimed at answering important questions such as
\begin{itemize}
\item Visualize forecasts of \profhit or other baselines and compare it with ground truth
at any node of the hierarchy
    \item Measure the performance of forecasts aggregated at any level of the hierarchy
    \item Visualize important parts of the hierarchy where there is significant performance difference or outliers.
    \item Provide a geographical view of performance across different countries.
\end{itemize}


\paragraph{Design methodology}
To visualize the improvements in performance between the DOW model and the \profhit model, a variety of technologies were considered.
We began with using the plotly library in python to create the visualizations.
This library allowed for the creation of custom plots and graphs and added a layer of interactivity.
Unfortunately, the plotly library only allowed for the existence of these plots within the code editor.
This was not an ideal method of sharing and interacting with the results of the experiments.
To further improve on the interactivity, usability, and sharebality, we moved to using Tableau\footnote{\url{https://www.tableau.com/}}.

Tableau allows for in-built and on-the-fly data visualizations that can fit any dataset. Tableau includes drag and drop features which makes editing visualizations a more time effective endeavor. 
It also allows for granular filtering and accessible data pop-ups for smooth and flexible 
interactions with visualizations enabling increased
insights at fine-grained levels.
We showcase the important visualizations we generated from tableau in Figure \ref{fig:viz}.
Each of the visualization has a filtering  feature (Figure \ref{fig:filter})
that allows the user to render the visualization at any level of the hierarchy.
The visualizations can be accessed by using the \href{https://www.tableau.com/products/viewer}{Tableau viewer}.\footnote{Demo available at: \url{https://www.dropbox.com/scl/fi/iq9c7coesxbsy9w2wk4t9/TableauOverview.mov?rlkey=sahbwwygrgbls0z1wduql9rlx&dl=0}}

One limitation of Tableau is that it does not allow for custom visualizations and users can only choose from the set of predefined visualization templates. 
Future work involves moving the visualizations to PowerBI and looking into custom plots.

% \begin{figure}[h]
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=0.2]{Images/WorldMap.png}
%         \caption{Robust Impact Visualizations with Data Pop-Ups}
%         \label{fig:enter-label}
%     \end{subfigure}
%     \begin{subfigure}
%         \centering
%         \includegraphics[scale=0.2]{Images/forecasts.png}
%         \caption{Visualize Forecasts with Errors and Ground Truth}
%         \label{fig:enter-label}
%     \end{subfigure}
% \end{figure}

